Planar Pixel Sensors for the ATLAS Upgrade: Beam Tests results

Results of beam tests with planar silicon pixel sensors aimed towards the ATLAS Insertable B-Layer and High Luminosity LHC (HL-LHC) upgrades are presented. Measurements include spatial resolution, charge collection performance and charge sharing between neighbouring cells as a function of track incidence angle for different bulk materials. Measurements of n-in-n pixel sensors are presented as a function of fluence for different irradiations. Furthermore p-type silicon sensors from several vendors with slightly differing layouts were tested. All tested sensors were connected by bump-bonding to the ATLAS Pixel read-out chip. We show that both n-type and p-type tested planar sensors are able to collect significant charge even after integrated fluences expected at HL-LHC.

==> newcommands.tex <==

\RequirePackage{xspace}

%\def \ninp {{\it n}-in-{\it p}}
\def \ninp {n-in-p}
%\def \ninn {{\it n}-in-{\it n}}
\def \ninn {n-in-n}
%\def \ntype {{\it n}-type}
\def \ntype {n-type}
%\def \ptype {{\it p}-type}
\def \ptype {p-type}

\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}


